Centroid Velocity Statistics of Molecular Clouds

We compute structure functions and Fourier spectra of 2D centroid velocity (CV) maps in order to study the gas dynamics of typical molecular clouds (MCs) in numerical simulations. We account for a simplified treatment of time-dependent chemistry and the non-isothermal nature of the gas and use a 3D radiative transfer tool to model the CO line emission in a post-processing step. We perform simulations using three different initial mean number densities of n_0 = 30, 100 and 300 cm^{-3} to span a range of typical values for dense gas clouds in the solar neighbourhood. We compute slopes of the centroid velocity increment structure functions (CVISF) and of Fourier spectra for different chemical components: the total density, H2 number density, 12CO number density as well as the integrated intensity of 12CO (J=1-0) and 13CO (J=1-0). We show that optical depth effects can significantly affect the slopes derived for the CVISF, which also leads to different scaling properties for the Fourier spectra. The slopes of CVISF and Fourier spectra for H2 are significantly steeper than those for the different CO tracers, independent of the density and the numerical resolution. This is due to the larger space-filling factor of H2 as it is better able to self-shield in diffuse regions, leading to a larger fractal co-dimension compared to CO.

==> journals.tex <==
%% journal abbreviations (from aastex.cls)

\def\jnl@style#1{{\rmfamily#1}}%
\def\jref@jnl#1{{\jnl@style#1}}%

\newcommand\aj{\jref@jnl{AJ}}%
          % Astronomical Journal
\newcommand\araa{\jref@jnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\jref@jnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\jref@jnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\jref@jnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\jref@jnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\jref@jnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\jref@jnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\jref@jnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\jref@jnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\jref@jnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\jref@jnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\jrasc{\jref@jnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\jref@jnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\jref@jnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\pra{\jref@jnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\jref@jnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\jref@jnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\jref@jnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\jref@jnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\jref@jnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasp{\jref@jnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\jref@jnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\jref@jnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\skytel{\jref@jnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\jref@jnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\jref@jnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\jref@jnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\jref@jnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\jref@jnl{Nature}}%
          % Nature
\newcommand\iaucirc{\jref@jnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\jref@jnl{Astrophys.~Lett.}}%
          % Astrophysics Letters
\newcommand\apspr{\jref@jnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\jref@jnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\jref@jnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\jref@jnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\jref@jnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\jref@jnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\jref@jnl{J.~Geophys.~Res.}}%
          % Journal of Geophysics Research
\newcommand\jqsrt{\jref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\jref@jnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\jref@jnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\jref@jnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\jref@jnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\jref@jnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\jref@jnl{Proc.~SPIE}}%
          % Proceedings of the SPIE

